Illusion Spaces in VR: The Interplay Between Size and Taper Angle Perception in Grasping

Leveraging the integration of visual and proprioceptive cues, research has uncovered various perception thresholds in VR that can be exploited to support haptic feedback for grasping. While previous studies have explored individual dimensions, such as size, the combined effect of multiple geometric properties on perceptual illusions remains poorly understood. We present a two-alternative forced choice study investigating the perceptual interplay between object size and taper angle. We introduce an illusion space model, providing detailed insights into how physical and virtual object configurations affect human perception. Our insights reveal how, for example, as virtual sizes increase, users perceive that taper angles increase, and as virtual angles decrease, users overestimate sizes. We provide a mathematical model of the illusion space, and an associated tool, which can be used as a guide for the design of future VR haptic devices and for proxy object selections.

==> section/2_RelatedWork.tex <==
\section{Related Work}

\add{When designing for advanced haptics in VR, researchers have to consider both co-location -- ensuring the haptic feedback is delivered in the correct location -- and object similarity -- ensuring the haptic feedback matches the shape properties of the virtual object ~\cite{propping}. In this section, we begin by discussing the different approaches to increasing haptic fidelity, before presenting the current knowledge in illusory techniques and the associated perceptual limits.}

\add{\subsection{Haptics in VR}}

Broadly, research has been exploring two avenues for achieving advanced haptics: (i) active haptics, and (ii) passive haptics. Active haptics leverage mechanical, actuated devices to carefully simulate virtual object properties during interaction. Passive haptics, conversely, use physical proxy objects in the user's vicinity, combined with visuo-proprioceptive illusions, to provide haptic counterparts for virtual objects. 

Active haptic devices have been demonstrated both for simulating co-location and similarity. An increasingly popular active approach for co-location, for example, includes encounter-type devices. These devices make the haptic surface available only 


\add{Researchers have been exploring advanced haptics devices in VR through two primary directions: (1) \textit{co-location (where)}: rendering haptics in different virtual object positions, through encounter-type devices or retargeting in passive haptics, e.g., ~\cite{follmer2013inform,azmandian2016haptic}.}, or (2) \textit{similarity (what)}: reflecting the properties of the virtual objects with controllers, wearable devices or resizing in passive objects, e.g., ~\cite{choi2016wolverine, bergstrom2019resized}.
% concentrating on providing haptics in VR via various devices. Some mechanically reflect the exact properties of the virtual objects (e.g., wearable haptic interface\cite{choi2016wolverine}) while others use proxy objects and illusions to render them (e.g., resized grasping\cite{bergstrom2019resized}). }

When illusions are applied within perceptual limits, users are considered unlikely to notice their occurrence. This makes studying these limits crucial to their success. \add{Although existing studies have estimated perceptual thresholds for grasping interactions, they have primarily focused on single geometric factor estimations. We turn our attention to multi-factor threshold estimation, to better understand how these factors impact one another. We begin by presenting the mainstream haptic designs and technologies, highlighting the role that illusions play in their feedback. We discuss the limitations of current illusion and perception studies.}





\add{Haptic devices have been developed to enhance user experience in VR interaction. To render haptics for \textit{co-location} tasks,} grounded and encounter-type platforms provide just-in-time feedback, that is only available at the exact moment the user needs it and can leave them otherwise hands-free. Examples of such devices include the commercially available Touch\footnote{3D Systems, USA - formerly Phantom from Sensable Technologies} and Omega\footnote{Force Dimension, Switzerland} devices, alongside research prototypes such as inFORM~\cite{follmer2013inform}, ShapeShift~\cite{siu2018shapeshift}, and REACH+~\cite{gonzalez2020reach+}. While high-resolution, inFORM, for example, features 30$\times$30 individually controllable haptic pins~\cite{follmer2013inform}. This resolution highlights how these devices are often mechanically complex, bulky, expensive, and necessitate a step towards infrastructuring that makes them impractical for everyday use. 
% Research has been exploring devices to add high-resolution haptic feedback to interactions in VR. 
\add{For the simulation of \textit{similarity} (specifically geometry and pressure) in grasping, much of this recent effort has focused on handheld and wearable device designs. These can be portable and are most akin to the controllers we see being adopted commercially. Prominent examples here include wearable controllers for grasping rigid objects~\cite{choi2016wolverine,choi2018claw}, axisymmetric devices for grasping pseudo-cylindrical objects~\cite{10.1145/3472749.3474782}, and multiple degree-of-freedom controllers for grasping asymmetric objects~\cite{ulan2024}. To date, however, these devices have remained specialist, cumbersome, and heavy. }
% Haptic devices have been developed to enhance user experience in VR interaction. Handheld and wearable controllers are popular and widely used. They offer a portable and easily integratable solution for incorporating haptic feedback into market controllers, enhancing user interaction and experience. \citet{choi2016wolverine} developed a low-cost lightweight wearable haptic device called Wolverine to simulate the grasping of rigid objects. They also designed a handheld VR controller called CLAW which supports grasping virtual objects, touching virtual surfaces, and triggering. ~\cite{choi2018claw} \citet{10.1145/3472749.3474782} introduced a hand-mounted shape display for grasping named X-Rings, enabling the users to grasp and release virtual objects while requiring it to be strapped to their hands. \citet{zhu2020fluidic} presented a new family of soft actuators referred to as fluidic fabric muscle sheets that can be used in wearable applications to exert force and contact the human body intimately. However, the handhold and wearable controllers often require users to hold or bear them, which adds weight burden and motion limitations to users.



% can change their properties to provide feedback and leave the users' hands free when interaction doesn't happen. 
% Some grounded devices are very accurate and able to provide a large range of force. Well-known commercial examples include Touch (3D Systems, USA - formerly Phantom from Sensable Technologies) and Omega (Force Dimension, Switzerland) ~\cite{adilkhanov2022haptic}. \citet{bau2010teslatouch} developed a touch screen called TeslaTouch that provides haptic feedback to fingers moving on the surface. Siu et al. developed a compact, high-resolution tabletop shape display called shaperShift which can be used for bimanual interaction. ~\cite{siu2018shapeshift} \citet{gonzalez2020reach+} proposed a REACH+ framework for dynamic visuo-haptic redirection with lower-speed but high-performance device. Although the grounded and encounter-type platforms can render some specific haptic feedback which is difficult for other devices, these platforms are often considered bulky, complex, and expensive.


% As a result of high-resolution active controllers remaining complex, specialist, and bespoke, 
\delete{Research has also been exploring opportunities for leveraging haptic illusions, both to extend the capacity of haptic controllers and to enable the use of physical objects around the user for feedback. \citet{ban2012modifying, ban2014displaying} proposed and validated a method to display various shapes with edges, curves, and surfaces with a simple physical device. \citet{zhao2018functional} further developed the method to extend haptic retargeting to complex, arbitrary shapes. \citet{bickmann2019haptic} showed that haptic feedback can be created by illusion without grasping any physical prop and developed a haptic illusion glove that can provide haptic feedback for various virtual objects such as a cup, a hammer, and a water can. 
\citet{kim2024big} use illusions in developing a fixed-sized controller leveraging finger-repositioning to create the illusion of dynamic size change. 
The perceived size of physical objects can be altered using illusions by distorting the visual object size~\cite{teng2018pupop}. In addition to direct hand interaction, \citet{yang2018vr} showed the perception can be influenced by illusion when visually changing the virtual tools (e.g. chopsticks) for interaction. These illusions seek to obscure visuo-proprioceptive mismatches to convince the user they are interacting with the virtual object when, in fact, they are interacting with \textit{something else}, potentially \textit{somewhere else}. }

\add{Apart from geometry and position rendering, haptic devices have been designed to render simulation of other aspects of \textit{similarity} such as textures~\cite{degraen2019enhancing, zhu2020fluidic,feick2023metareality}, temperatures~\cite{han2018haptic}, gravities~\cite{minamizawa2007gravity}, frictions~\cite{kim2022spinocchio}, etc.}

% another focus of haptic feedback is the texture simulation. \citet{degraen2019enhancing} developed 3D-printed hairs to infuence the feeling of roughness and hardness. \citet{zhu2020fluidic} presented a new family of soft actuators referred to as fluidic fabric muscle sheets that can be used in wearable applications to exert force and contact the human body intimately. MetaReality developed by \citet{feick2023metareality} can also alter their tactile surface properties upon lateral compression. 

\add{On the other hand, without the need for complex mechanical/electronic designs, passive haptics have the potential to render haptic feedback in a low-cost and much simpler way for both \textit{co-location (where)} and \textit{similarity (what)} tasks. Using passive haptic techniques has been proven effective in various environments and simulating virtual objects (e.g. kitchen\cite{hoffman1998physically}, ledge on the floor\cite{insko2001passive}, spiders~\cite{carlin1997virtual} and patients~\cite{kotranza2008virtual}). \citet{simeone2015substitutional} designed methods to leverage physical objects as VR haptic proxies and  \citet{zhu2019haptwist} further designed a construction toolkit to facilitate the creation of haptic devices. While being low-cost and giving realistic feedback of interacting with objects, passive haptics face the problem of low scalability and reusability. Recent research explored the possibility of addressing the shortages with illusions in visuo-haptic feedback.}



\add{\subsection{Illusions and Thresholds}}


\add{Due to the influence and application potentials of illusions in VR haptics, numerous studies have concentrated on exploring how illusions affect users' perceptions. This illusory work has one of two focuses: \textit{co-location} (\textit{where} the object is), or \textit{similarity} (\textit{what} the object is). }

\add{Illusions of \textit{co-location} have been heavily influenced by redirected touching~\cite{kohli2010redirected}, haptic retargeting~\cite{azmandian2016haptic} and haptic remapping \citet{lohse2019leveraging}.} These illusions seek to guide the user's physical hand towards a proxy object that is spatially decoupled from its virtual counterpart. Examples have demonstrated redirect controller buttons~\cite{zenner2019estimating,gonzalez2019investigating}, enabled users to grab objects placed around them~\cite{clarence2022investigating}, attempted to retarget random, unscripted reaches~\cite{clarence2021unscripted} and understanding the hand redirection illusions with multi-sensor data!\cite{feick2024predicting}. From work on these illusions, we have come to understand the spatial \textit{haptic coverage} of a physical object -- the area within which it can provide haptic feedback for virtual objects~\cite{clarence2024stacked}.

Illusions of \textit{similarity} largely explore the extent to which one physical object can feel like another. 
These illusions aim to convince users they are interacting with an object with one property (for example, a heavy hammer), while they in fact interact with an object with a different property or, at least, with an object with a different magnitude of that property (e.g., a lightweight bottle).
For example, illusions have been used to simulate factors in interaction such as geometry ~\cite{turchet2010influence}, force feedback ~\cite{lecuyer2000pseudo}, weight ~\cite{maehigashi2021virtual}, stiffness ~\cite{sanz2013elastic} and texture ~\cite{brahimaj2023cross}. 

To determine the limits of illusions in object perception, many studies have worked toward estimating the thresholds within which any difference between physical and virtual objects %can go reliably unnoticed
 cannot be reliably noticed. These limits now span a range of object properties (see Table \ref{tab:previousstudy}). For example, \citet{barbagli2006haptic} estimated the force-direction discrimination thresholds to be 31.9\textdegree{} when participants were given force-feedback with mismatched haptic and visual stimuli. \citet{hajnal2011perceptual} found users typically overestimated object slopes by around 6\textdegree{} without visual feedback.  
 \citet{auda2021enabling} found that participants do not perceive the size mismatch for virtual objects up to 50\% larger than the physical prop. They also found that different displacement had no influence on the results. \citet{bergstrom2019resized} estimated the thresholds of resizing virtual objects from physical objects. They found that size perception thresholds varied when the sizes of the physical objects changed, which showed the thresholds could be influenced by different conditions. The 3 cm wide cuboid could represent virtual ones from 2.7 cm to 4.4 cm, while the 9 cm cuboid was only able to represent virtual ones from 7 cm to 9.2 cm. 
 Similarly, \citet{de2019different} estimated the thresholds of discrimination of sizes, face orientations and curvatures in VR separately. The results show Just Noticeable Difference (JND) values of 5.75\%, 43.8\%, and 66.66\% of the physical objects for the width, orientation of the prism faces, and curvature of ellipsoid, respectively.

 \begin{table*}
  \caption{The perception limits of sizes and angles estimated by previous studies}
  \label{tab:previousstudy}

  \begin{tabular}{ll}
  
    \toprule
    \textbf{Study}&\textbf{Results}\\
    \hline
    \citet{barbagli2006haptic}&Force-direction threshold 31.9\textdegree{}\\
    \hline
    \citet{hajnal2011perceptual}&Overestimated the slope with fingers by around 6\textdegree{}\\
    \hline
    \citet{auda2021enabling}&Virtual size mismatch up to 50\% larger than the physical prop\\
    \hline
    \citet{bergstrom2019resized}&Physical size: 3 cm; virtual thresholds: 2.7 cm and 4.4 cm.\\ 
    &Physical size: 6 cm; virtual thresholds: 5.4 cm and 7.32 cm.\\
    &Physical size: 9 cm; virtual thresholds: 7.02 cm and 9.18 cm.\\
    \hline
    \citet{de2019different}\footnotemark[1]& Physical width: 4 cm; virtual thresholds: 3.77 cm and 4.55 cm\\
    &Physical angle: 10\textdegree{}; virtual thresholds: 5.62\textdegree{} and 14.56\textdegree{}\\
    &Physical curvature: 33 m$^{-1}$; virtual thresholds: 11 m$^{-1}$ and 47.08 m$^{-1}$\\
    \bottomrule
\end{tabular}
\end{table*}
\footnotetext[3]{The upscaling thresholds are derived theoretical values from their study results.}

 These previous studies have located the limits of illusions by carrying out one-dimensional estimation. They selected one property of an object and estimated the thresholds when illusions break in VR. 
 
 \add{ While estimated perception threshold values are given in these studies, their experimental settings seemingly caused differences in these values. In other words, changes in thresholds caused by other factors are not included in these contributions.}


 However, interplay exists in the perception of different properties. \add{In a scenario of virtual cooking class, \citet{feick2022designing} investigated the influence of grasping types, moving trajectories and object masses on user illusion detection out of the human operation habits of kitchen tools. They carried out user studies between these variables to find out if they limit or even extend the illusion space of user perception. In this study the frequentist analysis showed no significant interplay effect.} \citet{park2023visuo}, on the other hand, found an interplay between the primary moment and product of inertia (MOI and POI, which translates as differences in length and asymmetry) in the inertia tensor in handheld controllers. They proposed the models for haptic-to-visual (forward) matching, describing the virtual properties (MOI and POI) that best match a given physical object. They have also given the visual-to-haptic (inverse) equation for selecting haptic physical MOI and POI that best describe a given virtual object. This study suggests that the perception may vary in practice for objects with different properties. They concentrated on the best perceptual matching between virtual objects and physical proxy, while we aim at extending the physical objects' abilities to render haptics for more virtual ones by exploring the thresholds instead of best matching points (points of subjective equality).






 
 
 \add{While the previous studies acknowledged the value of studying the basic geometry features like size and angle, they rarely paid attention to this interplay. Varying object sizes directly impacts the joint orientations and torque forces experienced in the hand (primarily at the base of the fingers). Varying the shape of the object further alters the hand's pose, especially at the phalanges nearer the fingertips. It can also alter the direction of slippage at the fingertips and the direction of tangential forces applied by the fingers. Thus, both size and angles influence the grasping force and friction cones of the objects according to the analysis of grasping by \citet{zheng2022human}. These changes cannot be calculated or predicted from the previous reported results because they are single-variable studies (e.g., \citet{de2019different} studied size, angle and curvature but the results cannot be coupled because only one physical and virtual property was altered at the same time). Although it's impossible to study the perception in every different conditions, certain patterns and trends of how the factors interplay can be spotted. } How will the thresholds be influenced when multiple properties of the physical and virtual objects are incongruent at the same time? To answer these questions, we study multi-dimensional estimation of thresholds.
% \delete{Researchers have been concentrating on providing haptics in VR via active and passive controllers. Some mechanically reflect the exact properties of the virtual objects (active controllers, e.g., \citet{choi2016wolverine}) while others use proxy objects and illusions to render them (passive approaches, e.g., \citet{bergstrom2019resized}). 
% % Users may hardly notice the difference between incongruent physical and virtual conditions when illusion works in VR.
% When illusions are applied within perceptual limits, users are considered unlikely to notice their occurrence. This makes studying these limits crucial to their success.
% % Therefore, estimating the perception thresholds to test out when the illusions are strong enough to render realistic feedback is of great importance in haptic device designs. 
% Although existing studies have estimated perceptual thresholds for grasping interactions, they have primarily focused on single geometric factor estimations. We turn our attention to multi-factor threshold estimation, to better understand how these factors impact one another.
% % there are studies estimating perception thresholds in grasping tasks, they are however mostly limited to single-factor estimation. 
% We begin by presenting mainstream haptic device designs and technologies, highlighting the role that illusions play in their feedback. We discuss the limitations of current illusion and perception studies. }
% % and seek to propose an innovative model in this field. 
% % Based on this literature, we design our study on studying the interplay of size and shape in grasping to extend previous knowledge on perception thresholds.

% \delete{\subsection{Active Haptic Controllers for VR}

% %%haptic devices

% Research has been exploring devices to add high-resolution haptic feedback to interactions in VR. 
% Much of this recent effort has focused on handheld and wearable device designs. These can be portable and are most akin to the controllers we see being adopted commercially. Prominent examples here include wearable controllers for grasping rigid objects~\cite{choi2016wolverine,choi2018claw}, axisymmetric devices for grasping pseudo-cylindrical objects~\cite{10.1145/3472749.3474782}, and multiple degree-of-freedom controllers for grasping asymmetric objects~\cite{ulan2024}. To date, however, these controllers have remained specialist, cumbersome, and heavy. 
% % Haptic devices have been developed to enhance user experience in VR interaction. Handheld and wearable controllers are popular and widely used. They offer a portable and easily integratable solution for incorporating haptic feedback into market controllers, enhancing user interaction and experience. \citet{choi2016wolverine} developed a low-cost lightweight wearable haptic device called Wolverine to simulate the grasping of rigid objects. They also designed a handheld VR controller called CLAW which supports grasping virtual objects, touching virtual surfaces, and triggering. ~\cite{choi2018claw} \citet{10.1145/3472749.3474782} introduced a hand-mounted shape display for grasping named X-Rings, enabling the users to grasp and release virtual objects while requiring it to be strapped to their hands. \citet{zhu2020fluidic} presented a new family of soft actuators referred to as fluidic fabric muscle sheets that can be used in wearable applications to exert force and contact the human body intimately. However, the handhold and wearable controllers often require users to hold or bear them, which adds weight burden and motion limitations to users.

% On the other hand, grounded and encounter-type platforms provide just-in-time feedback, that is only available at the exact moment the user needs it and can leave them otherwise hands-free. Examples of such devices include the commercially available Touch\footnote{3D Systems, USA - formerly Phantom from Sensable Technologies} and Omega\footnote{Force Dimension, Switzerland} devices, alongside research prototypes such as inFORM~\citet{follmer2013inform}, ShapeShift~\cite{siu2018shapeshift}, and REACH+~\cite{gonzalez2020reach+}. While high-resolution, inFORM, for example, features 30$\times$30 individually controllable haptic pins~\cite{follmer2013inform}. This resolution highlights how these devices are often mechanically complex, bulky, expensive, and necessitate a step towards infrastructuring that makes them impractical for everyday use. 

% % can change their properties to provide feedback and leave the users' hands free when interaction doesn't happen. 
% % Some grounded devices are very accurate and able to provide a large range of force. Well-known commercial examples include Touch (3D Systems, USA - formerly Phantom from Sensable Technologies) and Omega (Force Dimension, Switzerland) ~\cite{adilkhanov2022haptic}. \citet{bau2010teslatouch} developed a touch screen called TeslaTouch that provides haptic feedback to fingers moving on the surface. Siu et al. developed a compact, high-resolution tabletop shape display called shaperShift which can be used for bimanual interaction. ~\cite{siu2018shapeshift} \citet{gonzalez2020reach+} proposed a REACH+ framework for dynamic visuo-haptic redirection with lower-speed but high-performance device. Although the grounded and encounter-type platforms can render some specific haptic feedback which is difficult for other devices, these platforms are often considered bulky, complex, and expensive.


% As a result of high-resolution active controllers remaining complex, specialist, and bespoke, research has also been exploring opportunities for leveraging haptic illusions, both to extend the capacity of haptic controllers and to enable the use of physical objects around the user for feedback. \citet{ban2012modifying, ban2014displaying} proposed and validated a method to display various shapes with edges, curves, and surfaces with a simple physical device. \citet{zhao2018functional} further developed the method to extend haptic retargeting to complex, arbitrary shapes. \citet{bickmann2019haptic} showed that haptic feedback can be created by illusion without grasping any physical prop and developed a haptic illusion glove that can provide haptic feedback for various virtual objects such as a cup, a hammer, and a water can. 
% \citet{kim2024big} use illusions in developing a fixed-sized controller leveraging finger-repositioning to create the illusion of dynamic size change. 
% The perceived size of physical objects can be altered using illusions by distorting the visual object size~\cite{teng2018pupop}. In addition to direct hand interaction, \citet{yang2018vr} showed the perception can be influenced by illusion when visually changing the virtual tools (e.g. chopsticks) for interaction. These illusions seek to obscure visuo-proprioceptive mismatches to convince the user they are interacting with the virtual object when, in fact, they are interacting with \textit{something else}, potentially \textit{somewhere else}. 

% % As a result of the potential, or even probable, mismatch between the locations and geometries of these objects, researchers use a range of illusions in order to make this haptic feedback `work'. 

% % Compared with other methods, illusion-based systems utilize physical objects to render various interaction options and stop fingers from intruding into the surface. If illusions are applied to passive physical objects, when interaction with the objects stops, users are free to continue other actions by putting the physical objects away. Therefore, haptic devices in VR benefit from exploring the influence, limits and mechanism of illusions. 
% }

% \delete{\subsection{Illusions in Haptic Feedback}


% %%studies of illusions, redirect, size (showing threshold)...
% Due to the influence and application potentials of illusions in VR haptics, numerous studies have concentrated on exploring how illusions affect users' perceptions. This illusory work has one of two focuses: \textit{where} the object is, or \textit{what} the object is. 

% Illusions of \textit{where} have been heavily influenced by redirected touching~\cite{kohli2010redirected} and haptic retargeting~\cite{azmandian2016haptic}. These illusions seek to guide the user's physical hand towards a proxy object that is spatially decoupled from its virtual counterpart. Examples have demonstrated redirect controller buttons~\citet{zenner2019estimating,gonzalez2019investigating}, enabled users to grab objects placed around them~\cite{clarence2022investigating}, and attempted to retarget random, unscripted reaches~\cite{clarence2021unscripted}. From work on these illusions, we have come to understand the spatial \textit{haptic coverage} of a physical object -- the area within which it can provide haptic feedback for virtual objects~\cite{clarence2024stacked}.

% Illusions of \textit{what} the object is largely explore the extent to which one physical object can feel like another. 
% These illusions aim to convince users they are interacting with an object with one property (for example, a heavy hammer), while they in fact interact with an object with a different property or, at least, with an object with a different magnitude of that property (e.g., a lightweight bottle).
% % One popular method to extend the application range of passive physical objects is to match physical objects with multiple virtual objects using illusions. Haptic illusions are caused by the differences between reality and perception, leading to changes in haptic experiences~\cite{kurzweg2024survey}. 
% % Many studies have concentrated on the pseudo-haptic feedback that physical objects can provide. 
% For example, illusions have been used to simulate factors in interaction such as geometry ~\cite{turchet2010influence}, force feedback ~\cite{lecuyer2000pseudo}, weight ~\cite{maehigashi2021virtual}, stiffness ~\cite{sanz2013elastic} and texture ~\cite{brahimaj2023cross}. 
% % Therefore, there have been many studies concentrating on illusions of object positions in VR, i.e. \textit{where} the object should be. \citet{kohli2010redirected} developed redirected touching, enabling one physical object to represent multiple differently shaped virtual objects. \citet{azmandian2016haptic} created a framework named haptic retargeting with which a single physical prop can provide haptics for multiple virtual objects. \citet{clarence2021unscripted, clarence2022investigating, clarence2024stacked} further increased the understanding in retargeting hand movements with illusions in VR. 
% % For interaction with physical objects, the haptic perception with users' hands influences the experience greatly. Hand movements help users to learn about the underlying representation of objects in memory and how the representation is derived and utilized~\cite{lederman1987hand}.
% % Different from \textit{where} the object is, studies on \textit{what} the object is explore the illusions on the objects' properties, mostly in hand-scale. 

% % In addition to studying the illusions themselves, 

% % Researchers have started to practically apply them in VR, too....
% %Researchers have begun to employ illusions on top of their active controller designs. Creating mechanical, actuated devices that can render a wide range of feedback and represent a broad array of virtual objects is challenging. As degrees of freedom, forces, surface orientations, etc., scale, so too does the mechanical complexity. Illusions may enhance the scope of this feedback. 
% % To address this issue, and attempt to limit or constrain this complexity, researchers have begun to consider employing illusions on top of their active controller designs. 
% % \citet{ban2012modifying, ban2014displaying} proposed and validated a method to display various shapes with edges, curves, and surfaces with a simple physical device. \citet{zhao2018functional} further developed the method to extend haptic retargeting to complex, arbitrary shapes. \citet{bickmann2019haptic} showed that haptic feedback can be created by illusion without grasping any physical prop and developed a haptic illusion glove that can provide haptic feedback for various virtual objects such as a cup, a hammer, and a water can. 
% % \citet{kim2024big} use illusions in developing a fixed-sized controller leveraging finger-repositioning to create the illusion of dynamic size change. 
% % The perceived size of physical objects can be altered using illusions by distorting the visual object size~\cite{teng2018pupop}. In addition to direct hand interaction, \citet{yang2018vr} showed the perception can be influenced by illusion when visually changing the virtual tools (e.g. chopsticks) for interaction.

% % We also study them aswell...
% %%just noticeable difference

% %%studies of angle perception. However, no threshold (stress resized again) means no standard.
%  To determine the limits of illusions in object perception, many studies have worked toward estimating the thresholds within which any difference between physical and virtual objects %can go reliably unnoticed
%  cannot be reliably noticed. These limits now span a range of object properties. For example, \citet{barbagli2006haptic} estimated the force-direction discrimination thresholds to be 31.9\textdegree{} when participants were given force-feedback with mismatched haptic and visual stimuli. \citet{hajnal2011perceptual} found users typically overestimated object slopes by around 6\textdegree{} without visual feedback.
%  % estimated human perception of angles of slopes using fingers. The participants were provided haptic feedback using a force-feedback device and could move their fingers to explore. They were then required to judge the angle in degrees verbally and the normal-sighted participants overestimated the slope by around 6\textdegree{}. This 
%  % this study did not offer corresponding visual feedback, which may yield different results if applied in VR.) 
%  % These studies concentrated on angle perception but can not be applied to VR applications because there were no corresponding virtual objects for visual feedback. And therefore, there were no visual stimuli to create illusions as it does in VR.
%  \citet{auda2021enabling} found that participants do not perceive the size mismatch for virtual objects up to 50\% larger than the physical prop. They also found that different displacement had no influence on the results. \citet{bergstrom2019resized} estimated the thresholds of resizing virtual objects from physical objects. They found that size perception thresholds varied when the sizes of the physical objects changed, which showed the thresholds could be influenced by different conditions. The 3 cm wide cuboid could represent virtual ones from 2.7 cm to 4.4 cm, while the 9 cm cuboid was only able to represent virtual ones from 7 cm to 9.2 cm. Similarly, \citet{de2019different} estimated the thresholds of discrimination of sizes, face orientations and curvatures in VR separately. The results show Just Noticeable Difference (JND) values of 5.75\%, 43.8\%, and 66.66\% of the physical objects for the width, orientation of the prism faces, and curvature of ellipsoid, respectively. %However, it's known that the thresholds change with conditions. The separately estimated thresholds have quite limited application values in practice.

%  \begin{table*}
%   \caption{Previous studies on perception of size and angle}
%   \label{tab:previousstudy}

%   \begin{tabular}{ll}
  
%     \toprule
%     \textbf{Study}&\textbf{Results}\\
%     \hline
%     \citet{barbagli2006haptic}&Force-direction threshold 31.9\textdegree{}\\
%     \hline
%     \citet{hajnal2011perceptual}&Overestimated the slope with fingers by around 6\textdegree{}\\
%     \hline
%     \citet{auda2021enabling}&Virtual size mismatch up to 50\% larger than the physical prop\\
%     \hline
%     \citet{bergstrom2019resized}&Physical size: 3 cm; virtual thresholds: 2.7 cm and 4.4 cm.\\ 
%     &Physical size: 6 cm; virtual thresholds: 5.4 cm and 7.32 cm.\\
%     &Physical size: 9 cm; virtual thresholds: 7.02 cm and 9.18 cm.\\
%     \hline
%     \citet{de2019different}\footnotemark[3]& Physical width: 4 cm; virtual thresholds: 3.77 cm and 4.55 cm\\
%     &Physical angle: 10\textdegree{}; virtual thresholds: 5.62\textdegree{} and 14.56\textdegree{}\\
%     &Physical curvature: 33 m$^{-1}$; virtual thresholds: 11 m$^{-1}$ and 47.08 m$^{-1}$\\
%     \bottomrule
% \end{tabular}
% \end{table*}
% \footnotetext[3]{The upscaling thresholds are derived theoretical values from their study results.}

%  These previous studies have located the limits of illusion by carrying out one-dimensional estimation, as listed in Table \ref{tab:previousstudy}. They selected one property of an object and estimated the thresholds when illusions break in VR.
%  % but for those properties which are not estimated, they are limited to certain constants. 
%  % The differences in the results show they are likely influenced by other factors in the studies. 
%  However, interplay exists in the perception of different properties. \citet{park2023visuo}, for example, found an interplay between the primary moment and product of inertia (MOI and POI, which translates as differences in length and asymmetry) in the inertia tensor in handheld controllers. They proposed the models for haptic-to-visual (forward) matching, describing the virtual properties (MOI and POI) that best match a given physical object. They have also given the visual-to-haptic (inverse) equation for selecting haptic physical MOI and POI that best describe a given virtual object. This study suggests that the perception may vary in practice for objects with different properties. They concentrated on the best perceptual matching between virtual objects and physical proxy, while we aim at extending the physical objects' abilities to render haptics for more virtual ones by exploring the thresholds instead of best matching points (points of subjective equality). When the sizes of the physical objects are different from previous studies, the perception threshold of the angle estimated by previous studies is likely to change because the direction of grasping force and finger span both change. And how will the thresholds be influenced when multiple properties of the physical and virtual objects are incongruent at the same time? To answer these questions, we study multi-dimensional estimation of thresholds.}




